Search for MeV Electron Recoils from Dark Matter in EXO-200

We present a search for electron-recoil signatures from the charged-current absorption of fermionic dark matter using the EXO-200 detector. We report an average electron recoil background rate of $6.8 \times 10^{-4}\, \mathrm{cts}\,\mathrm{kg}^{-1}\mathrm{yr}^{-1}\mathrm{keV}^{-1}$ above $4\,\mathrm{MeV}$ and find no statistically significant excess over our background projection. Using a total ${}^{136}\mathrm{Xe}$ exposure of $234.1\,\mathrm{kg}\,\mathrm{yr}$ we exclude new parameter space for the charged-current absorption cross-section for dark matter masses between $m_\chi = 2.6\,\mathrm{MeV} - 11.6\,\mathrm{MeV}$ with a minimum of $6\times 10^{-51}\,\mathrm{cm}^2$ at $8.3\,\mathrm{MeV}$ at the $90\%$ confidence level.

==> Dark Matter Paper EXO-200/authors.tex <==
\author{S.~Al~Kharusi}\affiliation{Physics Department, McGill University, Montreal, Quebec H3A 2T8, Canada}
\author{G.~Anton}\affiliation{Erlangen Centre for Astroparticle Physics (ECAP), Friedrich-Alexander-University Erlangen-N\"urnberg, Erlangen 91058, Germany}
\author{I.~Badhrees}\altaffiliation{Permanent address: King Abdulaziz City for Science and Technology, Riyadh, Saudi Arabia}\affiliation{Physics Department, Carleton University, Ottawa, Ontario K1S 5B6, Canada}
\author{P.S.~Barbeau}\affiliation{Department of Physics, Duke University, and Triangle Universities Nuclear Laboratory (TUNL), Durham, North Carolina 27708, USA}
\author{D.~Beck}\affiliation{Physics Department, University of Illinois, Urbana-Champaign, Illinois 61801, USA}
\author{V.~Belov}\affiliation{Institute for Theoretical and Experimental Physics named by A.I. Alikhanov of National Research Centre ``Kurchatov Institute'', Moscow 117218, Russia}\altaffiliation[Now a division of National Research Center ``Kurchatov Institute'', Moscow 123182, Russia]{}
\author{T.~Bhatta}\altaffiliation{Present address: Department of Physics and Astronomy, University of Kentucky, Lexington, Kentucky 40506, USA}\affiliation{Department of Physics, University of South Dakota, Vermillion, South Dakota 57069, USA}
\author{M.~Breidenbach}\affiliation{SLAC National Accelerator Laboratory, Menlo Park, California 94025, USA}
\author{T.~Brunner}\affiliation{Physics Department, McGill University, Montreal, Quebec H3A 2T8, Canada}\affiliation{TRIUMF, Vancouver, British Columbia V6T 2A3, Canada}
\author{G.F.~Cao}\affiliation{Institute of High Energy Physics, Beijing 100049, China}
\author{W.R.~Cen}\altaffiliation{Present address: Witmem Technology Co., Ltd., No.56 Beisihuan West Road, Beijing, China}\affiliation{Institute of High Energy Physics, Beijing 100049, China}
\author{C.~Chambers}\affiliation{Physics Department, McGill University, Montreal, Quebec H3A 2T8, Canada}
\author{B.~Cleveland}\altaffiliation{Also at SNOLAB, Sudbury, ON, Canada}\affiliation{Department of Physics, Laurentian University, Sudbury, Ontario P3E 2C6, Canada}
\author{M.~Coon}\affiliation{Physics Department, University of Illinois, Urbana-Champaign, Illinois 61801, USA}
\author{A.~Craycraft}\affiliation{Physics Department, Colorado State University, Fort Collins, Colorado 80523, USA}
\author{T.~Daniels}\affiliation{Department of Physics and Physical Oceanography, University of North Carolina at Wilmington, Wilmington, NC 28403, USA}
\author{L.~Darroch}\affiliation{Physics Department, McGill University, Montreal, Quebec H3A 2T8, Canada}
\author{S.J.~Daugherty}\altaffiliation{Present address: Carleton University, Ottawa, Ontario K1S 5B6, Canada}\affiliation{Physics Department and CEEM, Indiana University, Bloomington, Indiana 47405, USA}
\author{J.~Davis}\affiliation{SLAC National Accelerator Laboratory, Menlo Park, California 94025, USA}
\author{S.~Delaquis}\altaffiliation{Deceased}\affiliation{SLAC National Accelerator Laboratory, Menlo Park, California 94025, USA}
\author{A.~Der~Mesrobian-Kabakian}\altaffiliation{Present address: Commissariat \`a l'Energie Atomique et aux \'energies alternatives, France}\affiliation{Department of Physics, Laurentian University, Sudbury, Ontario P3E 2C6, Canada}
\author{R.~DeVoe}\affiliation{Physics Department, Stanford University, Stanford, California 94305, USA}
\author{J.~Dilling}\affiliation{TRIUMF, Vancouver, British Columbia V6T 2A3, Canada}
\author{A.~Dolgolenko}\affiliation{Institute for Theoretical and Experimental Physics named by A.I. Alikhanov of National Research Centre ``Kurchatov Institute'', Moscow 117218, Russia}
\author{M.J.~Dolinski}\affiliation{Department of Physics, Drexel University, Philadelphia, Pennsylvania 19104, USA}
\author{J.~Echevers}\affiliation{Physics Department, University of Illinois, Urbana-Champaign, Illinois 61801, USA}
\author{W.~Fairbank Jr.}\affiliation{Physics Department, Colorado State University, Fort Collins, Colorado 80523, USA}
\author{D.~Fairbank}\affiliation{Physics Department, Colorado State University, Fort Collins, Colorado 80523, USA}
\author{J.~Farine}\affiliation{Department of Physics, Laurentian University, Sudbury, Ontario P3E 2C6, Canada}
\author{S.~Feyzbakhsh}\affiliation{Amherst Center for Fundamental Interactions and Physics Department, University of Massachusetts, Amherst, MA 01003, USA}
\author{P.~Fierlinger}\affiliation{Technische Universit\"at M\"unchen, Physikdepartment and Excellence Cluster Universe, Garching 80805, Germany}
\author{Y.S.~Fu}\affiliation{Institute of High Energy Physics, Beijing 100049, China}
\author{D.~Fudenberg}\altaffiliation{Present address: Qventus, 295 Bernardo Ave, Suite 200, Mountain View, California 94043, USA}\affiliation{Physics Department, Stanford University, Stanford, California 94305, USA}
\author{P.~Gautam}\affiliation{Department of Physics, Drexel University, Philadelphia, Pennsylvania 19104, USA}
\author{R.~Gornea}\affiliation{Physics Department, Carleton University, Ottawa, Ontario K1S 5B6, Canada}\affiliation{TRIUMF, Vancouver, British Columbia V6T 2A3, Canada}
\author{G.~Gratta}\affiliation{Physics Department, Stanford University, Stanford, California 94305, USA}
\author{C.~Hall}\affiliation{Physics Department, University of Maryland, College Park, Maryland 20742, USA}
\author{E.V.~Hansen}\altaffiliation{Present address: Department of Physics at the University of California, Berkeley, California 94720, USA.}\affiliation{Department of Physics, Drexel University, Philadelphia, Pennsylvania 19104, USA}
\author{J.~Hoessl}\affiliation{Erlangen Centre for Astroparticle Physics (ECAP), Friedrich-Alexander-University Erlangen-N\"urnberg, Erlangen 91058, Germany}
\author{P.~Hufschmidt}\affiliation{Erlangen Centre for Astroparticle Physics (ECAP), Friedrich-Alexander-University Erlangen-N\"urnberg, Erlangen 91058, Germany}
\author{M.~Hughes}\affiliation{Department of Physics and Astronomy, University of Alabama, Tuscaloosa, Alabama 35487, USA}
\author{A.~Iverson}\affiliation{Physics Department, Colorado State University, Fort Collins, Colorado 80523, USA}
\author{A.~Jamil}\altaffiliation{Corresponding author: ako.jamil@yale.edu}\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut 06511, USA}
\author{C.~Jessiman}\affiliation{Physics Department, Carleton University, Ottawa, Ontario K1S 5B6, Canada}
\author{M.J.~Jewell}\altaffiliation{Present address: Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut 06511, USA}\affiliation{Physics Department, Stanford University, Stanford, California 94305, USA}
\author{A.~Johnson}\affiliation{SLAC National Accelerator Laboratory, Menlo Park, California 94025, USA}
\author{A.~Karelin}\affiliation{Institute for Theoretical and Experimental Physics named by A.I. Alikhanov of National Research Centre ``Kurchatov Institute'', Moscow 117218, Russia}
\author{L.J.~Kaufman}\altaffiliation{Also at Physics Department and CEEM, Indiana University, Bloomington, IN, USA}\affiliation{SLAC National Accelerator Laboratory, Menlo Park, California 94025, USA}
\author{T.~Koffas}\affiliation{Physics Department, Carleton University, Ottawa, Ontario K1S 5B6, Canada}
\author{R.~Kr\"{u}cken}\affiliation{TRIUMF, Vancouver, British Columbia V6T 2A3, Canada}
\author{A.~Kuchenkov}\affiliation{Institute for Theoretical and Experimental Physics named by A.I. Alikhanov of National Research Centre ``Kurchatov Institute'', Moscow 117218, Russia}
\author{K.S.~Kumar}\affiliation{Amherst Center for Fundamental Interactions and Physics Department, University of Massachusetts, Amherst, MA 01003, USA}
\author{Y.~Lan}\affiliation{TRIUMF, Vancouver, British Columbia V6T 2A3, Canada}
\author{A.~Larson}\affiliation{Department of Physics, University of South Dakota, Vermillion, South Dakota 57069, USA}
\author{B.G.~Lenardo}\affiliation{Physics Department, Stanford University, Stanford, California 94305, USA}
\author{D.S.~Leonard}\affiliation{IBS Center for Underground Physics, Daejeon 34126, Korea}
\author{G.S.~Li}\affiliation{Institute of High Energy Physics, Beijing 100049, China}
\author{S.~Li}\affiliation{Physics Department, University of Illinois, Urbana-Champaign, Illinois 61801, USA}
\author{Z.~Li}\altaffiliation{Present address: Physics Department, University of California, San Diego, La Jolla, CA 92093, USA}\affiliation{Institute of High Energy Physics, Beijing 100049, China}
\author{C.~Licciardi}\affiliation{Department of Physics, Laurentian University, Sudbury, Ontario P3E 2C6, Canada}
\author{Y.H.~Lin}\altaffiliation{Present address: Queen's University, Department of Physics, Engineering Physics \& Astronomy, Kingston, ON, Canada and SNOLAB, Sudbury, ON, Canada}\affiliation{Department of Physics, Drexel University, Philadelphia, Pennsylvania 19104, USA}
\author{R.~MacLellan}\altaffiliation{Present address: Department of Physics and Astronomy, University of Kentucky, Lexington, Kentucky 40506, USA}\affiliation{Department of Physics, University of South Dakota, Vermillion, South Dakota 57069, USA}
\author{T.~McElroy}\affiliation{Physics Department, McGill University, Montreal, Quebec H3A 2T8, Canada}
\author{T.~Michel}\affiliation{Erlangen Centre for Astroparticle Physics (ECAP), Friedrich-Alexander-University Erlangen-N\"urnberg, Erlangen 91058, Germany}
\author{B.~Mong}\affiliation{SLAC National Accelerator Laboratory, Menlo Park, California 94025, USA}
\author{D.C.~Moore}\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut 06511, USA}
\author{K.~Murray}\affiliation{Physics Department, McGill University, Montreal, Quebec H3A 2T8, Canada}
\author{O.~Njoya}\affiliation{Department of Physics and Astronomy, Stony Brook University, SUNY, Stony Brook, New York 11794, USA}
\author{O.~Nusair}\affiliation{Department of Physics and Astronomy, University of Alabama, Tuscaloosa, Alabama 35487, USA}
\author{A.~Odian}\affiliation{SLAC National Accelerator Laboratory, Menlo Park, California 94025, USA}
\author{I.~Ostrovskiy}\affiliation{Department of Physics and Astronomy, University of Alabama, Tuscaloosa, Alabama 35487, USA}
\author{A.~Perna}\affiliation{Department of Physics, Laurentian University, Sudbury, Ontario P3E 2C6, Canada}
\author{A.~Piepke}\affiliation{Department of Physics and Astronomy, University of Alabama, Tuscaloosa, Alabama 35487, USA}
\author{A.~Pocar}\affiliation{Amherst Center for Fundamental Interactions and Physics Department, University of Massachusetts, Amherst, MA 01003, USA}
\author{F.~Reti\`{e}re}\affiliation{TRIUMF, Vancouver, British Columbia V6T 2A3, Canada}
\author{A.L.~Robinson}\affiliation{Department of Physics, Laurentian University, Sudbury, Ontario P3E 2C6, Canada}
\author{P.C.~Rowson}\affiliation{SLAC National Accelerator Laboratory, Menlo Park, California 94025, USA}
\author{D.~Ruddell}\affiliation{Department of Physics and Physical Oceanography, University of North Carolina at Wilmington, Wilmington, NC 28403, USA}
\author{J.~Runge}\affiliation{Department of Physics, Duke University, and Triangle Universities Nuclear Laboratory (TUNL), Durham, North Carolina 27708, USA}
\author{S.~Schmidt}\affiliation{Erlangen Centre for Astroparticle Physics (ECAP), Friedrich-Alexander-University Erlangen-N\"urnberg, Erlangen 91058, Germany}
\author{D.~Sinclair}\affiliation{Physics Department, Carleton University, Ottawa, Ontario K1S 5B6, Canada}\affiliation{TRIUMF, Vancouver, British Columbia V6T 2A3, Canada}
\author{K.~Skarpaas}\affiliation{SLAC National Accelerator Laboratory, Menlo Park, California 94025, USA}
\author{A.K.~Soma}\affiliation{Department of Physics, Drexel University, Philadelphia, Pennsylvania 19104, USA}
\author{V.~Stekhanov}\affiliation{Institute for Theoretical and Experimental Physics named by A.I. Alikhanov of National Research Centre ``Kurchatov Institute'', Moscow 117218, Russia}
\author{M.~Tarka}\altaffiliation{Present address: SCIPP, University of California, Santa Cruz, CA, USA}\affiliation{Amherst Center for Fundamental Interactions and Physics Department, University of Massachusetts, Amherst, MA 01003, USA}
\author{S.~Thibado}\affiliation{Amherst Center for Fundamental Interactions and Physics Department, University of Massachusetts, Amherst, MA 01003, USA}
\author{M.~Todd}\affiliation{Physics Department, Colorado State University, Fort Collins, Colorado 80523, USA}
\author{T.~Tolba}\altaffiliation{Present address: Institute for Experimental Physics, Hamburg University, 22761 Hamburg, Germany}\affiliation{Institute of High Energy Physics, Beijing 100049, China}
\author{T.I.~Totev}\affiliation{Physics Department, McGill University, Montreal, Quebec H3A 2T8, Canada}
\author{R.H.M.~Tsang}\affiliation{Department of Physics and Astronomy, University of Alabama, Tuscaloosa, Alabama 35487, USA}
\author{B.~Veenstra}\affiliation{Physics Department, Carleton University, Ottawa, Ontario K1S 5B6, Canada}
\author{V.~Veeraraghavan}\altaffiliation{Present Address: Department of Physics and Astronomy, Iowa State University, Ames, IA 50011, USA}\affiliation{Department of Physics and Astronomy, University of Alabama, Tuscaloosa, Alabama 35487, USA}
\author{P.~Vogel}\affiliation{Kellogg Lab, Caltech, Pasadena, California 91125, USA}
\author{J.-L.~Vuilleumier}\affiliation{LHEP, Albert Einstein Center, University of Bern, Bern, Switzerland}
\author{M.~Wagenpfeil}\affiliation{Erlangen Centre for Astroparticle Physics (ECAP), Friedrich-Alexander-University Erlangen-N\"urnberg, Erlangen 91058, Germany}
\author{J.~Watkins}\affiliation{Physics Department, Carleton University, Ottawa, Ontario K1S 5B6, Canada}
\author{L.J.~Wen}\affiliation{Institute of High Energy Physics, Beijing 100049, China}
\author{U.~Wichoski}\affiliation{Department of Physics, Laurentian University, Sudbury, Ontario P3E 2C6, Canada}
\author{G.~Wrede}\affiliation{Erlangen Centre for Astroparticle Physics (ECAP), Friedrich-Alexander-University Erlangen-N\"urnberg, Erlangen 91058, Germany}
\author{S.X.~Wu}\altaffiliation{Present Address: Canon Medical Research US Inc., Vernon Hills, IL, USA}\affiliation{Physics Department, Stanford University, Stanford, California 94305, USA}
\author{Q.~Xia}\altaffiliation{Present address: Lawrence Berkeley National Laboratory, Berkeley, CA, USA}\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut 06511, USA}
\author{D.R.~Yahne}\affiliation{Physics Department, Colorado State University, Fort Collins, Colorado 80523, USA}
\author{L.~Yang}\affiliation{Physics Department, University of California, San Diego, La Jolla, CA 92093, USA}
\author{Y.-R.~Yen}\altaffiliation{Present address: Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA}\affiliation{Department of Physics, Drexel University, Philadelphia, Pennsylvania 19104, USA}
\author{O.Ya.~Zeldovich}\affiliation{Institute for Theoretical and Experimental Physics named by A.I. Alikhanov of National Research Centre ``Kurchatov Institute'', Moscow 117218, Russia}
\author{T.~Ziegler}\affiliation{Erlangen Centre for Astroparticle Physics (ECAP), Friedrich-Alexander-University Erlangen-N\"urnberg, Erlangen 91058, Germany}
